Estimating the Weight Enumerators of Reed-Muller Codes via Sampling

This paper develops an algorithmic approach for obtaining estimates of the weight enumerators of Reed-Muller (RM) codes. Our algorithm is based on a technique for estimating the partition functions of spin systems, which in turn employs a sampler that produces codewords according to a suitably defined Gibbs distribution. We apply our method to moderate-blocklength RM codes and derive approximate values of their weight enumerators. We observe that the rates of the weight enumerator estimates returned by our method are close to the true rates when these rates are either known or computable by brute-force search; in other cases, our computations provide provably robust estimates. As a byproduct, our sampling algorithm also allows us to obtain estimates of the weight spectra of RM codes. We illustrate our methods by providing estimates of the hitherto unknown weight enumerators of the RM$(11,5)$ code and the exact weight spectra of the RM$(10,3)$ and RM$(10,4)$ codes.

==> complexity.tex <==
\label{sec:complexity}

%Trash this! I'm not sure of these results.

In this section, we show that the counting problem of computing $A_{m,r}(\omega)$ is in general \#P-complete. Our proof strategy is to first transform our problem to an instance of counting the number of satisfying assignments in a constraint satisfaction problem (CSP). We first define the CSP of interest.

Fix the code RM$(m,r)$ with $m,r\geq 2$ and $r\leq m$ of dimension $k:=\binom{m}{\leq r}$ and a weight $0\leq \omega\leq 2^m=:n$. Let $H$ denote a parity-check matrix of the code with rows $\{\mathbf{h}_1,\ldots,\mathbf{h}_{n-k}\}$. We then define the following relations:
\begin{enumerate}
	\item The ``weight relation'' $\Gamma_\omega$, defined such that for any $\mathbf{x}\in \{0,1\}^n$, we have that $\mathbf{x}\in \Gamma_\omega$ iff $w_H(\mathbf{x}) = \omega$, and
	\item The ``parity-check relations'' $\Gamma_{\mathbf{h}_i}$, $1\leq i\leq n-k$, defined such that for any $\mathbf{x}\in \{0,1\}^n$, we have that $\mathbf{x}\in \Gamma_{\mathbf{h}_i}$ iff $\mathbf{h}_i^T \mathbf{x} = 0$  (over $\mathbb{F}_2$).
\end{enumerate}
Let $\Theta_\omega:= \{\mathbf{x}\in \{0,1\}^n: \mathbf{x}\in \Gamma_\omega\}$ and for $1\leq i\leq n-k$, let $\Theta_{\mathbf{h}_i}:= \{\mathbf{x}\in \{0,1\}^n: \mathbf{x}\in \Gamma_{\mathbf{h}_i}\}$. We then have that for $\mathcal{C}$ being RM$(m,r)$,
\[
\mathcal{C}_\omega = \Theta_\omega \cap \left(\bigcap_{i=1}^{n-k} \Theta_{\mathbf{h}_i}\right).
\]
This thus defines an instance of a constraint satisfaction problem, CSP$(\Gamma)$ as in \cite{chen1,chen2}, with $\Gamma = \{\Gamma_\omega, \Gamma_{\mathbf{h}_1},\ldots,\Gamma_{\mathbf{h}_{n-k}}\}$.
%\cite{dyerricherby}, with $\Gamma$ being the right-hand side above. 
Further, we have also shown that our problem of computing $A_{m,r}(\omega)$ is indeed the same as counting the number of satisfying assignments of the CSP above. In general, for any collection of relations as in \cite{chen1}, let \#CSP be the problem of counting the number of satisfying assignments, with \#CSP$(\Gamma)$ representing the corresponding problem for CSP$(\Gamma)$ as above.

We next briefly define the complexity classes P, NP (see \cite{arorabarak} for formal definitions) for decision problems and the complexity class FP for counting problems \cite{val1,val2}. For a given alphabet $\mathcal{X}$, let $\mathcal{X}^*:= \bigcup_{n\geq 0} \mathcal{X}^n$, where $\mathcal{X}^0$ is defined to be the empty symbol. Let $\Sigma = \{0,1\}$.

\begin{definition}
 A language $L\subseteq \Sigma^*$ is in the complexity class P iff there is a deterministic, polynomial-time Turing machine $M$ that outputs $1$ for all $x\in L$ and $0$ otherwise.
\end{definition}

\begin{definition}
	A language $L\subseteq \Sigma^*$ is in the complexity class NP if there is a deterministic, polynomial-time Turing machine $M$ (also called a \emph{verifier} for $L$) such that for every $x$, there exists a \emph{certificate} $u$ of length polynomial in the length of x such that $M(x,u) = 1$ iff $x\in L$, and $M(x,u) = 0$ for all $u$, otherwise.
\end{definition}

\begin{definition}
	Let $\Sigma$ be a finite alphabet. A function $f: \Sigma\to \mathbb{N}$ belongs to FP if there is a deterministic, polynomial time Turing machine $M$ that outputs $f(x)$, for any input $x\in \Sigma^*$.
\end{definition}

\begin{definition}
	Let $\Sigma$ be a finite alphabet. A function $f: \Sigma\to \mathbb{N}$ belongs to \#P if there is a polynomial time non-deterministic Turing machine $M$ such that, for any input $x\in \Sigma^*$, the number of accepting computations of $M$ on $x$ is exactly $f(x)$.
\end{definition}
%\begin{definition}
%	A function $f: \Sigma\to \mathbb{N}$ is \#P-complete if $f$ belongs to \#P and the computation of any function in \#P is polynomial time reducible to the computation of $f$.
%\end{definition}

It can easily be argued that our decision problem of deciding whether $A_{m,r}(\omega)>0$, or equivalently, of computing the weight spectrum at weight $\omega$ is in the class NP. Similarly, the counting problem of computing $A_{m,r}(\omega)$ is in the class \#P. Moreover, ``dichotomy results'' on the decision and counting complexities of CSPs are known:

\begin{theorem}[Schaefer's theorem \cite{schaefer}]
	\textsf{CSP} is either in P or is NP-complete.
\end{theorem}



\begin{theorem}[Thm. 21 in \cite{dyerricherby}]
	\#CSP is either computable in polynomial time or is \#P-complete.
\end{theorem}

We now show that the problem \#CSP$(\Gamma)$ defined above is in fact \#P-complete. To do so, we require some more definitions. Given $\Gamma$ as above and positive integers $i,j,\ell$ such that $i+j+\ell = n$, we define the $\{0,1\}^i\times \{0,1\}^j$ matrix $\mathsf{M}_{i,j,\ell}$ as follows: for $\mathbf{u}\in \{0,1\}^i$ and $\mathbf{v}\in \{0,1\}^j$, 
\[
\mathsf{M}_{i,j,\ell}(\mathbf{u},\mathbf{v}) := \left \lvert \{\mathbf{w}\in \{0,1\}^\ell: (\mathbf{u},\mathbf{v},\mathbf{w})\in \Gamma\} \right \rvert.
\]
In the above, we use the notation $(\mathbf{x},\mathbf{y})$ to denote the concatenation of vectors $\mathbf{x}$ and $\mathbf{y}$.

We then define the notion of a ``rectangular'' matrix, following \cite{dyerricherby}:
\begin{definition}
	An $p\times q$ matrix $B$ is rectangular if whenever $B_{s_1,t_1}, B_{s_1,t_2}, B_{s_2,t_1}>0$, we have that $B_{s_2,t_2}>0$.
\end{definition}
We then have the following theorem from \cite{dyerricherby}:
\begin{theorem}
	If $\mathsf{M}_{i,j,\ell}$ is not rectangular for every $i,j,\ell\geq 1$ such that $i+j+\ell = n$, then \#CSP$(\Gamma)$ is \#P-complete. 
\end{theorem}

Hence, all that we need to show is that there exists a choice of $\omega$, for $m,r\geq 2$, such that $\mathsf{M}_{i,j,\ell}$ is not rectangular, for some suitable $i,j,\ell\geq 1$ such that $i+j+\ell = n$.

\begin{proof}[Proof of Prop. III.1]
	Pick $\omega = n/4$ and $i=j=n/4$. Here, we must have $\ell = n/2$ so that $i+j+\ell = n$. Now, consider $\mathbf{u}_1 = 0^{n/4}$ and $\mathbf{u}_2 = 1^{n/4}$. Observe that $\mathsf{M}(\mathbf{u}_1,\mathbf{u}_1)>0$, since $0^{n/4}0^{n/4}1^{n/2} = \text{Eval}(x_1)\in \text{RM}(m,r)$. Similarly, $\mathsf{M}(\mathbf{u}_1,\mathbf{u}_2)>0$, since $0^{n/4}1^{n/4}0^{n/2} = \text{Eval}(x_2+x_1x_2)\in \text{RM}(m,r)$, and $\mathsf{M}(\mathbf{u}_2,\mathbf{u}_1)>0$, since $1^{n/4}0^{3n/4} = \text{Eval}(1+x_1+x_2+x_1x_2)\in \text{RM}(m,r)$. However, $\mathsf{M}(\mathbf{u}_2,\mathbf{u}_2) = 0$, since $w_H((\mathbf{u}_2,\mathbf{u}_2)) = n/2>n/4$. Hence, $\mathsf{M}_{n/4,n/4,n/2}$ is not rectangular, implying that \#CSP$(\Gamma)$ and hence our problem of computing $A_{m,r}(\omega)$ is \#P-complete.
\end{proof}
\textbf{The case $r=2$ is bothering me \ldots}

==> longtable.tex <==
\begin{center}
\begin{longtable}{|c | c}
        \hline 
       $\omega$ & $\frac{\log_2 \widehat{Z}}{2^m}$ \\ \hline 
        512 & 0.2967884396 \\ \hline
        516 & 0.3044142654 \\ \hline
        520 & 0.3098708781 \\ \hline
        524 & 0.3117907964 \\ \hline
        528 & 0.3159142454 \\ \hline
        532 & 0.3189211625 \\ \hline
        536 & 0.3210634545 \\ \hline
        540 & 0.3207781983 \\ \hline
        544 & 0.3292414942 \\ \hline
        548 & 0.3328099856 \\ \hline
        552 & 0.3325168244 \\ \hline
        556 & 0.33856337 \\ \hline
        560 & 0.3386807389 \\ \hline
        564 & 0.3458428641 \\ \hline
        568 & 0.3445511304 \\ \hline
        572 & 0.3516682886 \\ \hline
        576 & 0.3508534035 \\ \hline
        580 & 0.3532623147 \\ \hline
        584 & 0.3584547222 \\ \hline
        588 & 0.3586827759 \\ \hline
        592 & 0.3643411714 \\ \hline
        596 & 0.3626564667 \\ \hline
        600 & 0.3667665428 \\ \hline
        604 & 0.3719335599 \\ \hline
        608 & 0.369610572 \\ \hline
        612 & 0.3721375515 \\ \hline
        616 & 0.3791433248 \\ \hline
        620 & 0.378965573 \\ \hline
        624 & 0.3822856786 \\ \hline
        628 & 0.3860521584 \\ \hline
        632 & 0.3867559043 \\ \hline
        636 & 0.3904530961 \\ \hline
        640 & 0.3904831381 \\ \hline
        644 & 0.3886726124 \\ \hline
        648 & 0.3947849511 \\ \hline
        652 & 0.3994320755 \\ \hline
        656 & 0.4002439455 \\ \hline
        660 & 0.4041690765 \\ \hline
        664 & 0.405357908 \\ \hline
        668 & 0.4046384939 \\ \hline
        672 & 0.4083316113 \\ \hline
        676 & 0.4066164489 \\ \hline
        680 & 0.4122257465 \\ \hline
        684 & 0.416757749 \\ \hline
        688 & 0.4154593686 \\ \hline
        692 & 0.4151373483 \\ \hline
        696 & 0.4193250188 \\ \hline
        700 & 0.4228290541 \\ \hline
        704 & 0.426700815 \\ \hline
        708 & 0.4232395375 \\ \hline
        712 & 0.4260621686 \\ \hline
        716 & 0.4285488693 \\ \hline
        720 & 0.4313321598 \\ \hline
        724 & 0.4340572763 \\ \hline
        728 & 0.4378637509 \\ \hline
        732 & 0.4374155272 \\ \hline
        736 & 0.439222757 \\ \hline
        740 & 0.4383031672 \\ \hline
        744 & 0.4420132493 \\ \hline
        748 & 0.4419631323 \\ \hline
        752 & 0.4488207103 \\ \hline
        756 & 0.44347076 \\ \hline
        760 & 0.4476962448 \\ \hline
        764 & 0.4495450293 \\ \hline
        768 & 0.4489722934 \\ \hline
        772 & 0.4509841781 \\ \hline
        776 & 0.454131732 \\ \hline
        780 & 0.4562743742 \\ \hline
        784 & 0.4541577203 \\ \hline
        788 & 0.45629281 \\ \hline
        792 & 0.4579614556 \\ \hline
        796 & 0.4595784776 \\ \hline
        800 & 0.4604385389 \\ \hline
        804 & 0.4628383539 \\ \hline
        808 & 0.4655936825 \\ \hline
        812 & 0.4666761093 \\ \hline
        816 & 0.4660395012 \\ \hline
        820 & 0.4687878527 \\ \hline
        824 & 0.4677889949 \\ \hline
        828 & 0.4692737546 \\ \hline
        832 & 0.470439285 \\ \hline
        836 & 0.4720260806 \\ \hline
        840 & 0.4757967321 \\ \hline
        844 & 0.4728329498 \\ \hline
        848 & 0.4764918242 \\ \hline
        852 & 0.4758886476 \\ \hline
        856 & 0.4780183181 \\ \hline
        860 & 0.4790559436 \\ \hline
        864 & 0.4783843133 \\ \hline
        868 & 0.4801069772 \\ \hline
        872 & 0.4827332212 \\ \hline
        876 & 0.4821388907 \\ \hline
        880 & 0.4821725246 \\ \hline
        884 & 0.4830228041 \\ \hline
        888 & 0.4833586871 \\ \hline
        892 & 0.4838592857 \\ \hline
        896 & 0.4842506892 \\ \hline
        900 & 0.4869631419 \\ \hline
        904 & 0.4878321476 \\ \hline
        908 & 0.4893220263 \\ \hline
        912 & 0.4883336432 \\ \hline
        916 & 0.4889590025 \\ \hline
        920 & 0.4889086859 \\ \hline
        924 & 0.4898091244 \\ \hline
        928 & 0.491859122 \\ \hline
        932 & 0.4903585543 \\ \hline
        936 & 0.4922892439 \\ \hline
        940 & 0.4914607835 \\ \hline
        944 & 0.4934381041 \\ \hline
        948 & 0.4931433172 \\ \hline
        952 & 0.4945423179 \\ \hline
        956 & 0.4929904748 \\ \hline
        960 & 0.4943895946 \\ \hline
        964 & 0.4952178539 \\ \hline
        968 & 0.4945798255 \\ \hline
        972 & 0.495527873 \\ \hline
        976 & 0.4970328654 \\ \hline
        980 & 0.4966750273 \\ \hline
        984 & 0.4954571397 \\ \hline
        988 & 0.4963111889 \\ \hline
        992 & 0.4968925105 \\ \hline
        996 & 0.4972624121 \\ \hline
        1000 & 0.496628302 \\ \hline
        1004 & 0.4974914362 \\ \hline
        1008 & 0.4975938289 \\ \hline
        1012 & 0.4975072018 \\ \hline
        1016 & 0.4966127403 \\ \hline
        1020 & 0.4978946567 \\ \hline
        1024 & 0.4980060621 \\ \hline
    \caption{Table of estimates $\frac{\log_2 \widehat{Z}}{2^m}$ of the rates of the weight enumerators for the RM$(11,5)$ code, for weights $\omega = 512, 516, 520, ..., 1024$. Here, the parameters $\tau = 1\times 10^6$, $t=10$, and $\delta = 0.001$.} \label{tab:rmwt115}\\
\end{longtable}
\end{center}

==> wtdist.tex <==
In Section \ref{sec:estimate}, we discussed a technique to obtain estimates of the sizes of (potentially arbitrarily-)constrained subcodes of RM codes. In this section, we restrict our attention to the constant weight constraint; in other words, we shall concern ourselves in this section to exact computation of the weight distribution of RM codes, algorithmically. While our interest is primarily on RM codes, our exposition here applies to arbitrary linear codes that are constructed using the Plotkin $(\mathbf{u} , \mathbf{u}+\mathbf{v})$ construction.

Consider a pair $\cC_0 \subseteq \cC$ of nested linear codes over $\F_2$ \footnote{The results in this section are applicable for any field $\F_q$.} (observe that the RM family of codes obeys such a nesting property; in particular, RM$(m,r-1)\subseteq \text{RM}(m,r)$, for $m\geq 1$ and $1\leq r\leq m$). Let  $\cC_0, \cC_1,\ldots,\cC_{M-1}$ be an enumeration of the cosets of $\cC_0$ in $\cC$, where $M = |\cC/\cC_0| = 2^{\dim\cC - \dim \cC_0}$. 

Let $A_{\cC}(z)$ and $A_{\cC_i}(z)$ denote the weight enumerator polynomials of $\cC$ and $\cC_i$, respectively. Since $\cC$ is the disjoint union of the $\cC_i$s, we have
$$
A_{\cC}(z) = \sum_{i=0}^{M-1} A_{\cC_i}(z).
$$

Let $\overline{\cC}$ be the code obtained from $\cC$ and $\cC_0$ using the $(\u , \u+\v)$ construction:
$$
\overline{\cC} = \{(\u,\u+\v) : \u \in \cC, \v \in \cC_0\}.
$$

\begin{lemma}
	\label{lem:1}
	The weight enumerator of $\overline{\cC}$ is given by
	$$
	A_{\overline{\cC}}(z) = \sum_{i=0}^{M-1} {(A_{\cC_i}(z))}^2.
	$$
\end{lemma}
\begin{proof}
	We only need the observation that for any $\u \in \cC$ and $\v \in \cC_0$, $\u$ and $\u+\v$ belong to the same coset $\cC_i$. 
	Thus,
	\begin{align*}
		A_{\overline{\cC}}(z) &= \sum_{\u \in \cC} \sum_{\v \in \cC_0} z^{w_H(\u,\u+\v)} \\
		&= \sum_{i=0}^{M-1} \sum_{\u \in \cC_i} \sum_{\v \in \cC_0} z^{w_H(\u)} z^{w_H(\u+\v)} \\
		&= \sum_{i=0}^{M-1} \sum_{\u \in \cC_i} z^{w_H(\u)} \sum_{\mathbf{v'} \in \cC_i} z^{w_H(\mathbf{v'})} \\
		&= \sum_{i=0}^{M-1} A_{\cC_i}(z) \cdot A_{\cC_i}(z).
	\end{align*}
\end{proof}

In the case of Reed-Muller codes, we have a situation such as the following: there is a nested sequence of codes $\cC_{00} \subset \cC_0 \subset \cC$, and another nested pair $\overline{\cC}_0 \subset \overline{\cC}$ such that $\overline{\cC}_0$ (resp. $\overline{\cC}$) is obtained from $\cC_{00}$ and $\cC_0$ (resp.\ $\cC_0$ and $\cC$) via the $(u \mid u+v)$ construction:
$$
\overline{\cC}_0 = \{(u,u+v) : u \in \cC_0, v \in \cC_{00}\}  \ \ \text{ and } \ \  \overline{\cC} = \{(u,u+v) : u \in \cC, v \in \cC_0\}.
$$
In this terminology, $\cC_{00}, \cC_0,$ and $\cC$ can respectively be associated with RM$(m,r-2)$, RM$(m,r-1)$ and RM$(m,r)$, and then $\overline{\cC}_0 = \text{RM}(m+1,r-1)$ and $\overline{\cC} = \text{RM}(m+1,r)$, where $m\geq 1$ and $2\leq r\leq m$.
We show below that the weight enumerator polynomial of a coset of $\overline{\cC}_0$ in $\overline{\cC}$ is computable from the weight enumerators of the cosets of $\cC_{00}$ in $\cC$.

We introduce some convenient notation first. Let $M$ and $M_0$ be the size of the quotient spaces $\cC/\cC_0$ and $\cC_0/\cC_{00}$, respectively, so that $M \cdot M_0$ is the size of $\cC / \cC_{00}$. Enumerate the cosets of $\cC_0$ in $\cC$ as $\cC_0, \cC_1, \ldots, \cC_{M-1}$, and those of $\cC_{00}$ in $\cC_0$ as $\cC_{00}, \cC_{01}, \ldots, \cC_{0,M_0-1}$. We extend this to a listing, $\cC_{ij}$, $i = 0,1,\ldots,M-1$, $j = 0,1,\ldots,M_0-1$, of the cosets of $\cC_{00}$ in $\cC$ as follows: if $\cC_i = \mathbf{u'} + \cC_0$ and $\cC_{0j} = \mathbf{v'} + \cC_{00}$ for some $\mathbf{u'} \in \cC$ and $\mathbf{v'} \in \cC_0$, then $\cC_{ij} = \mathbf{u'}+\mathbf{v'}+\cC_{00}$. With this, we have $\cC_{ij} \subset \cC_i$ for all $i,j$. Recall that $\cC/\cC_0$ and $\cC_0/\cC_{00}$ are $\F_q$-vector spaces. The induced vector space structure on $\cC / \cC_{00}$ is such that for all $\a, \b \in \F_q$, we have $\a \cdot \cC_{ij} + \b \cdot \cC_{kl} = \cC_{st}$ iff $\a \cdot \cC_i + \b \cdot \cC_k = \cC_s$ and $\a \cdot \cC_{0j} + \b \cdot \cC_{0l} = \cC_{0t}$.

As usual, let $A_{\cC_i}(z)$ and $A_{\cC_{ij}}(z)$ denote the weight enumerators of $\cC_i$ and $\cC_{ij}$, respectively.
\begin{lemma}
	\label{lem:2}
	Let $\u \in \cC$ and $\v \in \cC_0$ be given, so that $(\u,\u+\v) \in \overline{\cC}$ and $[\u,\u+\v]  := (\u,\u+\v) + \overline{\cC}_0$ is a coset of $\overline{\cC}_0$ in $\overline{\cC}$. Let $\cC_i := \u + \cC_0$ and $\cC_{0j} = \v + \cC_{00}$. Then, the weight enumerator of $[\u,\u+\v]$ is given by
	$$
	A_{[\u,\u+\v]}(z)  \ = \ \sum_{l=0}^{M_0-1} A_{\cC_{il}}(z) \cdot A_{\cC_{il} + \cC_{0j}}(z) 
	$$
\end{lemma}
\begin{proof}
	Observe that the set $\cC_i$ is the union of all the disjoint sets $\cC_{il}$ where $0\leq l\le M_0 -1 $.
	Thus,
	\begin{align*}
		A_{[u,u+v]}(z) &= \sum_{\c \in \cC_0} \sum_{\mathbf{c'} \in \cC_{00}} z^{w_H(\u+\c,\u+\v+\c+\mathbf{c'})} \\
		&= \sum_{l=0}^{M_0-1} \sum_{\mathbf{c''} \in \cC_{il}} \sum_{\mathbf{c'} \in \cC_{00}} z^{w_H(\mathbf{c''})} z^{w_H(\mathbf{c''}+\v+\mathbf{c'})} \\
		&= \sum_{l=0}^{M_0-1} \sum_{\u \in \cC_{il}} z^{w_H(\mathbf{c''})} \sum_{\x \in \cC_{il} + \cC_{0j}} z^{w_H(\x)} \\
		&= \sum_{l=0}^{M_0-1} A_{\cC_{il}}(z) \cdot A_{\cC_{il} + \cC_{0j}}(z)
	\end{align*}
\end{proof}
\section{Simplifying Computations Using the Automorphism Group}
Consider now the computation of weight distributions of binary Reed-Muller (RM) codes. First, for some preliminaries. Recall that RM codes of blocklength $2^m$ consist of the evaluations of multilinear polynomials $f\in \mathbb{F}_2[x_1,\ldots,x_m]$ over vertices of the $m$-dimensional unit hypercube. In particular, the $r^{\text{th}}$-order binary RM code RM$(m,r)$ can be written as
\[
\text{RM}(m,r) = \{\text{Eval}(f): f\in \mathbb{F}_2[x_1,\ldots,x_m] \text{ and deg}(f)\leq r \},
\]
where we use the notation Eval$(f):= \left(f({y}): {y} = (y_1,\ldots,y_m) \in \{0,1\}^m\right)$, with the coordinates ${y} = (y_1,\ldots,y_m)$ being ordered according to the standard lexicographic ordering. Moreover, given $f\in \mathbb{F}_2[x_1,\ldots,x_m]$, we define deg$(f)$ to be the largest degree of a monomial present in $f$. 

From the definition above, the following facts can be deduced (see Chapter 13 of \cite{mws}): the dimension dim$(\text{RM}(m,r)) = {m\choose [0:r]}$, where we use the notation ${n\choose [a:b]}$ to mean $\sum_{i=a}^{b} {n\choose i}$, for $a\leq b$. Further, RM$(m,r)\subset \text{RM}(m,r^\prime)$, for $0\leq r< r^\prime\leq m$, and any codeword ${c}\in \text{RM}(m,r)$ can be written as the concatenation ${c} = \left(u \mid u+v\right)$, where $u\in \text{RM}(m-1,r)$ and $v\in \text{RM}(m-1,r-1)$, for $r\leq m-1$. This hence means that Lemmas \ref{lem:1} and \ref{lem:2} can be employed to compute the weight distributions of RM codes, in a recursive manner, by computing the weight distributions of cosets of one RM code within another.

Now, following \cite{yao}, we show that the weight distributions of certain cosets of RM$(m,r)$ in RM$(m,r^\prime)$, for $r<r^\prime$, are equal. First, let us define the coset
\[
\cC_f:= \text{Eval}(f) + \text{RM}(m,r),
\]
of RM$(m,r)$ in RM$(m,r^\prime)$, where $\text{deg}(f)\leq r^\prime$. %is such that all monomials in its (unique) expansion have their degrees in $[r+1:r^\prime]$. 
Further, for any $p\in \mathbb{F}_2[x_1,\ldots,x_m]$, we define the set $\cM_p:= p+\text{span}(\{g\in \mathbb{F}_2[x_1,\ldots,x_m]:\ \text{deg}(g)\leq r\})$. It is easy to check that all the cosets of RM$(m,r)$ in RM$(m,r^\prime)$ can be written as $\cC_f$ for some $f$, and that the words in $\cC_f$ are evaluations of the polynomials in the set $\cM_f$. Also, it is sufficient to restrict attention to those $\cC_f$ where $f$ is such that all monomials in its (unique) expansion have their degrees in $[r+1:r^\prime]$.

Second, we recall another important property of RM codes, which is the structure of its automorphism group. Recall that if $S_N$ is the symmetric group on $N$ elements, the automorphism group of a length-$N$ code $\cC$ is given by
\[
\text{Aut}(\cC) = \{\pi\in S_N: \pi(c)\in \cC, \text{ for all } c\in \cC\}.
\]
Consider the general affine group GA$(m,2)$ consisting of affine permutations $(A,b)$ of $m$-tuples $y = (y_1,\ldots,y_m)\in \{0,1\}^m$, given by the maps
\[
y \mapsto Ay + b,\ A\in \mathbb{F}_2^{m\times m},\ b\in \mathbb{F}_2^m,
\]
where the matrix $A$ is invertible. It is well-known (see, for example, Theorem 24 in \cite[Chapter 13]{mws}) that Aut$(\text{RM}(m,r)) = \text{GA}(m,2)$, for all $1\leq r\leq m-2$, and Aut$(\text{RM}(m,r))= S_{2^m}\supset \text{GA}(m,2)$, for $r\in \{0,m-1,m\}$. Now, for a polynomial $f \in \mathbb{F}_2[x_1,\ldots,x_m]$, we define $(A,b)\cdot f:= \left(f(Ay+b): y \in \{0,1\}^m\right)$ to be the action of the permutation $(A,b)\in \text{GA}(m,2)$ on $f$. The action of $(A,b)$ on a subset $X\subseteq \mathbb{F}_2[x_1,\ldots,x_m]$, written as $(A,b)\cdot X$, can be defined similarly to be the set of actions of $(A,b)$ on the polynomials in $X$.

Now, observe that for $(A,b)\in \text{GA}(m,2)$, and for $f$ such that deg$(f)\leq r^\prime$, 
\begin{align*}
	(A,b)\cdot \cM_f &= (A,b)\cdot f + \text{span}(\{g:\ \text{deg}(g)\leq r\})\\
	&= h + \text{span}(\{g:\ \text{deg}(g)\leq r\}) = \cM_h,
\end{align*}
for $h = (A,b)\cdot f\in \mathbb{F}_2[x_1,\ldots,x_m]$. Note that the first equality holds since the vector space $\text{span}(\{g:\ \text{deg}(g)\leq r\})$ is invariant under the action of $(A,b)$. It can be argued that deg$(h)\leq r^\prime$, and hence that the evaluations of polynomials in $\cM_h$ give rise to a coset of RM$(m,r)$ in RM$(m,r^\prime)$. Finally, since permutations of coordinates preserve the weights of words, and hence the weight distribution of cosets, it holds that the weight enumerator polynomials $A_{\cC_f}(z)$ and $A_{\cC_h}(z)$, where $h = (A,b)\cdot f$, are equal.
